Towards Unified Dialogue System Evaluation: A Comprehensive Analysis of Current Evaluation Protocols

As conversational AI-based dialogue management has increasingly become a trending topic, the need for a standardized and reliable evaluation procedure grows even more pressing. The current state of affairs suggests various evaluation protocols to assess chat-oriented dialogue management systems, rendering it difficult to conduct fair comparative studies across different approaches and gain an insightful understanding of their values. To foster this research, a more robust evaluation protocol must be set in place. This paper presents a comprehensive synthesis of both automated and human evaluation methods on dialogue systems, identifying their shortcomings while accumulating evidence towards the most effective evaluation dimensions. A total of 20 papers from the last two years are surveyed to analyze three types of evaluation protocols: automated, static, and interactive. Finally, the evaluation dimensions used in these papers are compared against our expert evaluation on the system-user dialogue data collected from the Alexa Prize 2020.

==> figure/static_corr.tex <==

\begin{figure}[htb]
    \centering
    \includegraphics[trim=50 50 50 50, clip, width=\columnwidth]{img/correlation_results_expert.pdf}
    \caption{Correlations between the 8 dialogue dimensions from the expert evaluation.}
    \label{fig:corr}
\end{figure}

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=\linewidth]{img/correlation_results_interact.png}
%    \caption{Correlations between dialogue evaluation dimensions from the static evaluation. Axis labels follow that of Figure 1.}
%    \label{fig:corr_inter}
%\end{figure}

==> table/extra.tex <==
\begin{table*}[htbp!]
\centering

\begin{subtable}{\textwidth}
\centering\small
    \begin{tabular}{c|l}
    \hline
    \multirow{4}{*}{\tt Fluency}
    & Whether the response from the listener is understandable \cite{lin_moel_2019} \\ \cline{2-2}
    % & Did the language seem accurate? & \\ 
    & Whether the response is fluent and natural \cite{li_incremental_2019} \\ \cline{2-2}
    & Whether each sentence has correct grammar \cite{luo_auto-encoder_2018} \\ \cline{2-2}
    & Fluency measures if the produced response itself is fluent \cite{wu_proactive_2019}: \\
    \hline
    \tt Consistency
    & Whether the reply is fluent and grammatical \cite{li_syntactically_2018} \\ \hline
    \tt Readability
    & Whether the utterance is grammatically formed \cite{qiu_are_2019} \\ \hline
    \tt Grammaticality
    & Whether the response is fluent and grammatical \cite{zhu_retrieval-enhanced_2019} \\ \hline
    \end{tabular}
\caption{Grammatical Capability}
\label{tab:grammar}
\end{subtable}

\begin{subtable}{\textwidth}
\centering\resizebox{\textwidth}{!}{
    \begin{tabular}{c|l}
    \hline
    \multirow{3}{*}{\tt Relevance}
        & Whether the responses of the listener seem appropriate to the conversation \cite{lin_moel_2019} \\ \cline{2-2}
        % & Were they on-topic? & \\
        & Whether the response is appropriate/relevant in the current context language \cite{moghe_towards_2018} \\ \cline{2-2}
        & Whether the reply is relevant to the query \cite{qiu_are_2019} \\ \hline
    \tt Appropriateness
        & Whether the response is appropriate in grammar, topic, and logic \cite{young_augmenting_2018} \\ \hline
    \multirow{2}{*}{\tt Coherence}
        & Whether the generated response is relevant to the input \cite{luo_auto-encoder_2018} \\ \cline{2-2}
        & Whether the whole dialogue is fluent (does not contain irrelevant or illogical responses)  \cite{wu_proactive_2019} \\
         \hline
    \tt Context Coherence
        & Whether the response is coherent with the context and guides the following utterances \cite{li_incremental_2019} \\ \hline
    \tt Logic
        & Whether the post and the reply are logically matched \cite{li_syntactically_2018} \\\hline
    \tt Sensibleness
        & Whether the response makes sense given the context \cite{adiwardana_towards_2020} \\ \hline
        % & , ...If anything seems off — confusing, illogical, out of context, or factually wrong — then it should be labeled as, 'does not make sense'" & \\
    \end{tabular}}
\caption{Turn Coherence}
\label{tab:coherence}
\end{subtable}

\begin{subtable}{\textwidth}
\centering\resizebox{\textwidth}{!}{
    \begin{tabular}{c|l}
    \hline
    \multirow{4}{*}{\tt Informativeness}
        & Whether the response provides new information and knowledge in addition to the post \cite{young_augmenting_2018} \\ \cline{2-2}
        & Whether the response has unique words and multi-topic clauses \cite{tian_learning_2019} \\ \cline{2-2}
        % & - 1: universal response/response containing no more than 3 unique words \\
        % & - 2: normal response of a single clause or a single topic \\
        % & - 3: informative response with at least two clauses of different topics, which transfer the current \\
        % & $\quad\:\,$ conversation to another scenario \\
        & Whether the response has meaningful information relevant to its message \cite{zhu_retrieval-enhanced_2019} \\ \cline{2-2}
        & Whether the model makes full use of knowledge in the response \cite{wu_proactive_2019}\\ \hline
    \multirow{2}{*}{\tt Specificity}
        & Whether the model produced movie-specific responses or generic responses \cite{moghe_towards_2018} \\ \cline{2-2}
        & Whether the response is specific to the context \cite{adiwardana_towards_2020} \\ \hline
        % & the reply should not be able to be used in dozens of different contexts \\
    \tt Diversity
        & Whether the reply narrates with diverse words \cite{qiu_are_2019} \\ \hline
    \end{tabular}}
\caption{Response Informativeness}
\label{tab:specificity}
\end{subtable}

\caption{Grammatical Capability}
\label{tbl:dimension-groups}
\end{table*}

% \input{table/grammaticality_reduction}
% \input{table/relevance_reduction}
% \input{table/informativeness_reduction}

==> table/grammaticality_reduction.tex <==

\begin{table}[htb!]
\centering\small \resizebox{\columnwidth}{!}{
\begin{tabular}{c|l}
\bf Metric & \MC{c}{Definition} \\
\hline\hline
\multirow{4}{*}{Fluency}
    & Whether the response from the listener is \\
    & understandable [11] \\ \cline{2-2}
    & Whether the response is fluent and natural [10] \\ \cline{2-2}
    & Whether each sentence has correct grammar [3] \\ \cline{2-2}
    & Whether the produced response itself is \\
    & fluent [15] \\
    \hline
Consistency
    & Whether the reply is fluent and grammatical [1] \\ \hline
Readability
    & Whether the utterance is grammatically \\
    & formed [13] \\ \hline
Grammaticality
    & Whether the response is fluent and \\
    & grammatical [18] \\
\end{tabular}}
\caption{Grammatical Capability}
\label{tab:grammar}
\end{table}

==> table/informativeness_reduction.tex <==

\begin{table}[htb!]
\centering\resizebox{\columnwidth}{!}{
\begin{tabular}{c|l}
\bf Metric & \MC{c}{Definition} \\
\hline\hline
\multirow{4}{*}{Informativeness}
    & Whether the response provides new information \\
    & and knowledge in addition to the post [7] \\ \cline{2-2}
    & Whether the response has unique words and \\
    & multi-topic clauses [14] \\ \cline{2-2}
    & Whether the response has meaningful information \\
    & relevant to its message [18] \\ \cline{2-2}
    & Whether the model makes full use of knowledge \\
    & in the response [15]\\ \hline
\multirow{2}{*}{Specificity}
    & Whether the model produced movie-specific \\
    & responses or generic responses [4] \\ \cline{2-2}
    & Whether the response is specific \\
    & to the context [20] \\ \hline
Diversity
    & Whether the reply narrates with diverse words [13] \\
\end{tabular}}
\caption{Response Informativeness}
\label{tab:specificity}
\end{table}

==> table/relevance_reduction.tex <==

\begin{table}[htb!]
\centering\resizebox{\columnwidth}{!}{
\begin{tabular}{c|l}
\bf Metric & \MC{c}{Definition} \\
\hline\hline
\multirow{3}{*}{Relevance}
    & Whether the responses of the listener seem  \\
    & appropriate to the conversation [11] \\ \cline{2-2}
    & Whether the response is appropriate/relevant \\
    & in the current context language [4] \\ \cline{2-2}
    & Whether the reply is relevant to the query [13] \\ \hline
Appropriateness
    & Whether the response is appropriate \\
    & in grammar, topic, and logic [7] \\ \hline
\multirow{3}{*}{Coherence}
    & Whether the generated response is relevant \\
    & to the input [3] \\ \cline{2-2}
    & Whether the whole dialogue does not contain \\
    & irrelevant or illogical responses  [15] \\
     \hline
Context Coherence
    & Whether the response is coherent with the \\
    & context and guides the following utterances [10] \\ \hline
Logic
    & Whether the post and the reply are logically \\
    & matched [1] \\\hline
Sensibleness
    & Whether the response makes sense given the \\
    & context [20] \\
\end{tabular}}
\caption{Response Relevance}
\label{tab:coherence}
\end{table}

==> tex/relatedwork.tex <==
\section{Related Work}

The evaluation of open-domain chat-oriented dialogue agents has commonly been accomplished through the use of automated metrics and human evaluation \cite{du2019boosting,lin_moel_2019,li_diversity-promoting_2016,wang_improving_2019,tian_learning_2019}. Although it has been noted that human users provide the ultimate authority on whether the goals of the conversation with a dialogue agent were achieved \cite{ghandeharioun_approximating_2019}, automated metrics are often used as a supplementary metric due to the greater expense in obtaining human evaluations and the lack of standardized evaluation procedure for such human evaluations, which makes it challenging to compare different works to one another. However, for automated metrics to be an appropriate measure of dialogue system quality, they would need to be shown to be good approximations of human evaluations. As \newcite{liu_how_2016} show, commonly used automated metrics like BLEU and embedding-based similarity measures actually correlate weakly at best with human judgements, thus suggesting that most automated evaluations are poor evaluation metrics at this point. 

\newcite{du2019boosting} use a static human evaluation where human annotators choose the preferred response between multiple options, in which the response options are produced by randomly sampling a single turn of dialogue from the test set and the subsequent response is generated from the system. Similarly, \newcite{lin_moel_2019} use a static evaluation method as well, but on top of choosing the preferred response between multiple options, the human annotators are instructed to also give a rating on a scale of 1 to 5 for three dialogue dimensions: empathy, relevancy, and fluency. \newcite{lian2019learning} forgo the preference selection method completely for their static evaluation in favor of a rating scale; however, their human annotators are instructed to give a rating of either 0, 1, or 2 for a single, generic quality dimension. Although each of these works uses a similar static evaluation procedure, it is clear that their evaluation dimensions are not the same, which does little to alleviate the difficulty in comparing systems to one another when evaluated in such an ad-hoc manner. Additionally, such a static evaluation does not allow for the true capability of dialogue agents to be adequately assessed, since it ensures the system is operating in a non-dynamic environment. This prevents the system from being evaluated in a realistic multi-turn setting, in which its repetitive, self-inconsistent, or error-handling qualities would be revealed. 

Even for those works that have conducted an online, interactive human evaluation, the evaluation dimensions are also inconsistent with one another. \newcite{zhang_personalizing_2018} and \newcite{ghandeharioun_approximating_2019} both use such an evaluation, but evaluate on different dimensions - fluency, consistency, and engagingness vs fluency, relatedness, quality, diversity, and empathy, respectively - and even on different scales - 1 to 5 vs 1 to 7, respectively. Without a standard protocol for dialogue evaluations, it is near impossible to accumulate cross-work comparisons and assess the progress of the field.
